An Alternative Prior Process for Nonparametric Bayesian Clustering

Prior distributions play a crucial role in Bayesian approaches to clustering. Two commonly-used prior distributions are the Dirichlet and Pitman-Yor processes. In this paper, we investigate the predictive probabilities that underlie these processes, and the implicit "rich-get-richer" characteristic of the resulting partitions. We explore an alternative prior for nonparametric Bayesian clustering -- the uniform process -- for applications where the "rich-get-richer" property is undesirable. We also explore the cost of this process: partitions are no longer exchangeable with respect to the ordering of variables. We present new asymptotic and simulation-based results for the clustering characteristics of the uniform process and compare these with known results for the Dirichlet and Pitman-Yor processes. We compare performance on a real document clustering task, demonstrating the practical advantage of the uniform process despite its lack of exchangeability over orderings.

==> macros.tex <==
\newcommand{\comment}[1]{}

% just to help while drafting the paper
\usepackage{color}
\newcommand{\todo}{\textcolor{red}}

\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\blambda{\boldsymbol{\lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bomega{\boldsymbol{\omega}}
\def\bphi{\boldsymbol{\phi}}
\def\bpi{\boldsymbol{\pi}}
\def\bTheta{\boldsymbol{\Theta}}

\def\ba{\boldsymbol{a}}   
\def\bb{\boldsymbol{b}}   
\def\bc{\boldsymbol{c}}   
\def\bbf{\boldsymbol{f}}   
\def\bg{\boldsymbol{g}}   
\def\bm{\boldsymbol{m}}   
\def\bn{\boldsymbol{n}}   
\def\bp{\boldsymbol{p}}   
\def\bq{\boldsymbol{q}}   
\def\bu{\boldsymbol{u}}   
\def\bw{\boldsymbol{w}}   
\def\bx{\boldsymbol{x}}   
\def\by{\boldsymbol{y}}   
\def\bz{\boldsymbol{z}}   
\def\bzero{\boldsymbol{0}}
\def\bA{\boldsymbol{A}}   
\def\bB{\boldsymbol{B}}   
\def\bC{\boldsymbol{C}}   
\def\bH{\boldsymbol{H}}   
\def\bI{\boldsymbol{I}}   
\def\bN{\boldsymbol{N}}   
\def\bQ{\boldsymbol{Q}}   
\def\bX{\boldsymbol{X}}   
\def\bZ{\boldsymbol{Z}}   
\def\bS{\boldsymbol{S}}   

\def\g{\,|\,}   

\newcommand{\is}{:=}

\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}

